DynamiTe: Dynamic Termination and Non-termination Proofs

There is growing interest in termination reasoning for non-linear programs and, meanwhile, recent dynamic strategies have shown they are able to infer invariants for such challenging programs. These advances led us to hypothesize that perhaps such dynamic strategies for non-linear invariants could be adapted to learn recurrent sets (for non-termination) and/or ranking functions (for termination). In this paper, we exploit dynamic analysis and draw termination and non-termination as well as static and dynamic strategies closer together in order to tackle non-linear programs. For termination, our algorithm infers ranking functions from concrete transitive closures, and, for non-termination, the algorithm iteratively collects executions and dynamically learns conditions to refine recurrent sets. Finally, we describe an integrated algorithm that allows these algorithms to mutually inform each other, taking counterexamples from a failed validation in one endeavor and crossing both the static/dynamic and termination/non-termination lines, to create new execution samples for the other one.

==> alg.tex <==



\section{Algorithm}
%
%\begin{center}
%\begin{program}[style=tt]
%  DynCategorize(Program) : (phi\_term, phi\_nonterm, phi\_unknown) \{ 
%  itraces = gen\_rand\_inp(Program)
%  
%  whi\tab le depth < UPPERBOUND:
%      term\_base\_inp, term\_inp, mayloop\_inp = partition(itraces)
%      valid\_rcs, nt\_cex = prove\_NonTerm(mayloop\_inp)
%      term\_pre, valid\_ranking\_funcs, t\_cex = prove\_Term(term\_base\_inp, term\_inp)
%      itraces = gen\_traces(nt\_cex, t\_cex)
%      if n\tab ot itraces or (term\_pre \/ valid\_rcs = TRUE):
%          break;
%      depth++; \untab
%      
%  \}
%\end{program}
%\end{center}

\red{chanh to update}

==> cfa.tex <==

\begin{definition}[Control-flow automaton~\cite{Henzinger2002}]
A (deterministic) \emph{control flow automaton} denoted $\aut$, is a
tuple $\aut = \langle Q, q_0, X, s, \cfarightarrow{\,} \rangle$ where $Q$ is a
finite set of control locations and $q_0$ is the initial control location, $X$
is a finite sets of typed variables, $s$ is the statement language 
and $\cfarightarrow{\,}\subseteq Q \times s \times Q$ is a finite set
of labeled edges.
\end{definition}

\noindent
We will use the follow statement language:
\[\begin{array}{lll}
  % \mid \ttite{b}{e}{e} 
  e &::=& e \oplus e \mid  c \mid \mathbb{Z} \mid x\\
  b &::=& b \otimes b \mid \textsf{true} \mid \neg b \\
  s &::=& s \texttt{ ; } s \mid x := e \mid \ttassume{b} \mid \ttskip
\end{array}\]


\paragraph{Valuations and semantics.}
We define a \emph{valuation} of variables 
$\vln : X \rightarrow \mathit{Val}$ to be a mapping from
variable names to values. Let $\Vlns$ be the set of all valuations.
%
The notation $\vln' \in \sem{s}\vln$ means that executing statement $s$, using
the values given in $\vln$, leads to a new
valuation $\vln'$, mapping variables $X$ to new values. Notations $\sem{e}\vln$ and $\sem{b}\vln$ represent side-effect free numeric and boolean valuations, respectively.
%
We assume that for every $\vln,s$, that $\sem{s}\vln$ is computed in finite time.
%
The automaton edges, along with $\sem{s}$, give rise to possible transitions, denoted
$(q,\vln) \cfarightarrow{s} (q',\vln')$ (we omit these rules for lack of space.

A \emph{run} of a CFA is an alternation of automaton states and
valuations: $\run=q_0,\vln_0,q_1,\vln_1,q_2,\dots$
such that $\forall i \geq0.\ (q_i,\vln_i) \cfarightarrow{s} (q_{i+1},\vln_{i+1})$.
%\paragraph{Safety and termination.}
%
We say that CFA $\aut$ can \emph{reach} automaton state $q$ (\emph{safety}) provided that
there exists a run $\run= q_0,\vln_0,q_1,\vln_1,...$ such that there is
some $i \geq 0 $ such that  $q_i=q$.
%
%We say that CFA $\aut$ \emph{terminates} provided that there
%are no infinite runs.
%$\forall q_0,\vln_0,q_1,\vln_1,...\in\Pi(\aut)$ such that there is
%some $i \geq 0 $ such that  $q_i=q$.

\begin{definition}[Induced transition system]
For CFA $\aut=  \langle Q, q_0, s, X, \cfarightarrow{ } \rangle$,
with 
% crash script \crasht\ and
valuation space $\Vlns$, we define the \emph{induced transition system}
$M^q_\aut = \langle \states_\aut, \labels_\aut, \trans_\aut,
\sigma^0_\aut \rangle$ as:
\[ \begin{array}{rl}
    \states_\aut =& \Vlns \circ (\{pc\} \rightarrow Q),\\
    \labels_\aut =& s, \\
    \trans_\aut =& \{
          \vln[pc\mapsto q], s, \vln'[pc\mapsto q']
          \mid  q\cfarightarrow{s}q' \;\wedge\; \sem{s}\theta = \theta' \},\\
    \sigma^0_\aut =& \vln_o[pc \mapsto q_0]
\end{array} \]
where $\vln_0$ associates variables with initial dummy values,
and $\vln[pc \mapsto q]$ means the extension of $\vln$ so that it maps $pc$ to $q$. 
%
We will simply write $M_\aut$ when we mean $M^{q_0}_\aut$.
For a run $\run = q_0,\vln_0,q_1,\vln_1,\dots$ of $\aut$, we define the 
\emph{induced trace} to be
%\[\begin{array}{rl}
%$$\pi_\run \equiv \langle q_0,\vln_0 \rangle, s_0, \langle q_1,\vln_1 \rangle, s_1,\dots$$
$$\pi_\run \equiv \vln_0[pc\mapsto q_0], \vln_1[pc\mapsto q_1], \dots$$
where
$\forall i\geq 0. \exists s.
( \vln_i[pc\mapsto q_i], s, \vln_{i+1}[pc\mapsto q_{i+1}])
\in \trans_\aut$. 
%\end{array}\]

\end{definition}

==> instrument.tex <==
%!TEX root = ./paper.tex

\section{Instrumentation for Dynamic Analysis}



==> nla-term.tex <==
\texttt{bresenham1} &            & $-c, -c + k                                $ & 20.4     &     \rTRUE & 7.1   &     \rTRUE & 27.8  &     \rTRUE \\ 
\texttt{cohencu1  } & cubic sum  & $k + -z                                    $ & 2.5      &     \rTRUE & 4.0   &     \rTRUE & 6.8   &     \rTRUE \\ 
\texttt{cohencu2  } & cubic sum  & $k + -z, k + -y                            $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{cohencu3  } & cubic sum  & $-x, k + -x                                $ & 2.2      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{cohencu4  } & cubic sum  & $-n + 2\cdot k                             $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{cohencu5  } & cubic sum  & $                                          $ & 0.0      &      \rUNK & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{cohencu6  } & cubic sum  & $-x + y, a + -n                            $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{cohencu7  } & cubic sum  & $-n + -x + 57\cdot y, a + -n               $ & 8.6      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{dijkstra1 } & square root & $n + -q                                    $ & 1.5      &     \rTRUE & 5.8   &     \rTRUE & 7.6   &     \rTRUE \\ 
\texttt{dijkstra2 } & square root & $-c + k                                    $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{dijkstra3 } & square root & $-c + k                                    $ & 6.3      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{dijkstra4 } & square root & $h, -c, q, -c + k                          $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{dijkstra5 } & square root & $-c + k                                    $ & 14.4     &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{dijkstra6 } & square root & $-c + k                                    $ & 6.6      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{divbin1   } & int div    & $                                          $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{egcd      } & gcd        & $q, r, a, b                                $ & 5.8      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{egcd2     } & gcd        & $                                          $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{egcd3     } & gcd        & $v, -37\cdot b + -d, \mathit{(et\ al.)}$ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{fermat1   } & product    & $                                          $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{freire1   } & square root & $                                          $ & 0.0      &      \rUNK & 13.2  &      \rUNK & 13.9  &      \rUNK \\ 
\texttt{geo1      } & geo series & $ x + -y, y, \mathit{(et\ al.)} $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{geo2      } & geo series & $k + -c                                    $ & 15.8     &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{geo3      } & geo series & $-x, k + -c                                $ & 5.7      &     \rTRUE & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{hard      } & int div    & $                                          $ & 20.0     &       \rAF & \rTO  &      \rUNK & 898.6 &       \rAF \\ 
\texttt{hard2     } & int div    & $p                                         $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{knuth     } & product    & $                                          $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{knuth-nosqrt} &            & $                                          $ & 7.7      &      \rUNK & \rTO  &      \rUNK & \rTO  &      \rUNK \\ 
\texttt{lcm1      } & divisor    & $                                          $ & 0.0      &      \rUNK & 8.7   &      \rUNK & 8.9   &      \rUNK \\ 
\texttt{lcm2      } & divisor    & $y                                         $ & 0.1      &     \rTRUE & 6.7   &      \rUNK & 7.1   &      \rUNK \\ 
\texttt{mannadiv  } &            & $y3                                        $ & \rUNK    &     \rTRUE & \rUNK &      \rUNK & 0.0   &        UNK \\ 
\texttt{prod4br   } & gcd, lcm   & $b, a                                      $ & \rUNK    &     \rTRUE & \rTO  &      \rUNK & \rTO  &        UNK \\ 
\texttt{prodbin   } & gcd, lcm   & $                                          $ & \rAF     &       \rAF & \rAF  &       \rAF & \rAF  &       \rAF \\ 
\texttt{ps2       } & pow sum    & $k + -c                                    $ & 3.9      &     \rTRUE & 5.0   &     \rTRUE & 9.1   &     \rTRUE \\ 
\texttt{ps3       } & pow sum    & $k + -c                                    $ & 4.3      &     \rTRUE & 8.8   &     \rTRUE & 13.4  &     \rTRUE \\ 
\texttt{ps4       } & pow sum    & $k + -c                                    $ & 4.8      &     \rTRUE & 9.6   &     \rTRUE & 14.7  &     \rTRUE \\ 
\texttt{ps5       } & pow sum    & $k + -c                                    $ & 4.9      &     \rTRUE & 7.4   &     \rTRUE & 12.5  &     \rTRUE \\ 
\texttt{ps6       } & pow sum    & $k + -c                                    $ & 4.8      &     \rTRUE & 28.8  &     \rTRUE & 33.8  &     \rTRUE \\ 
\texttt{sqrt1     } & square root & $-c, k + -c                                $ & 7.0      &     \rTRUE & 173.9 &     \rTRUE & 181.3 &     \rTRUE \\ 

==> nladigbench.tex <==
\texttt{bresenham1} &            & $-c, -c + k  $ & 20.42 &     \rTRUE & 7.05 &     \rTRUE & 29.66 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-bresenham1-both-t.c.log 
\texttt{cohencu1  } & cubic sum  & $k + -z      $ & 2.54 &     \rTRUE & 3.99 &     \rTRUE & 8.53 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu1-both-t.c.log 
\texttt{cohencu2  } & cubic sum  & $k + -z, k + -y$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu2-both-t.c.log 
\texttt{cohencu3  } & cubic sum  & $-x, k + -x  $ & 2.16 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu3-both-t.c.log 
\texttt{cohencu4  } & cubic sum  & $-n + 2\cdot k$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu4-both-t.c.log 
\texttt{cohencu5  } & cubic sum  & $            $ & 0.00 &    \nparse & 10993.45 &    \nparse & 9.33 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu5-both-t.c.log 
\texttt{cohencu6  } & cubic sum  & $-x + y, a + -n$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu6-both-t.c.log 
\texttt{cohencu7  } & cubic sum  & $-n + -x + 57\cdot y, a + -n$ & 8.58 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-cohencu7-both-t.c.log 
\texttt{dijkstra1 } & square root & $n + -q      $ & 1.50 &     \rTRUE & 5.83 &     \rTRUE & 9.39 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra1-both-t.c.log 
\texttt{dijkstra2 } & square root & $-c + k      $ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra2-both-t.c.log 
\texttt{dijkstra3 } & square root & $-c + k      $ & 6.34 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra3-both-t.c.log 
\texttt{dijkstra4 } & square root & $h, -c, q, -c + k$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra4-both-t.c.log 
\texttt{dijkstra5 } & square root & $-c + k      $ & 14.35 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra5-both-t.c.log 
\texttt{dijkstra6 } & square root & $-c + k      $ & 6.63 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-dijkstra6-both-t.c.log 
\texttt{divbin1   } & int div    & $            $ & 0.00 &    \nparse & 0.00 &    \nparse & 1.71 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-divbin1-both-t.c.log 
\texttt{egcd      } & gcd        & $q, r, a, b  $ & 5.77 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-egcd-both-t.c.log 
\texttt{egcd2     } & gcd        & $            $ & 0.00 &    \nparse & 0.00 &    \nparse & 1.80 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-egcd2-both-t.c.log 
\texttt{egcd3     } & gcd        & $c + -v, v, -37\cdot b + -d, -293\cdot b + -d, -2341\cdot b + -d, -18725\cdot b + -d, -37449\cdot b + c + -d, 10083\cdot c + -d, 322639\cdot c + -d, 2581111\cdot c + -d, -1677722\cdot b + -d$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-egcd3-both-t.c.log 
\texttt{fermat1   } & product    & $            $ & 0.00 &    \nparse & 0.00 &    \nparse & 2.49 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-fermat1-both-t.c.log 
\texttt{freire1   } & square root & $            $ & 0.00 &    \nparse & 13.18 &    \nparse & 15.91 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-freire1-both-t.c.log 
\texttt{geo1      } & geo series & $c + -x, -c + x, -y, x + -y, y, k + -c$ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-geo1-both-t.c.log 
\texttt{geo2      } & geo series & $k + -c      $ & 15.80 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-geo2-both-t.c.log 
\texttt{geo3      } & geo series & $-x, k + -c  $ & 5.72 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-geo3-both-t.c.log 
\texttt{hard      } & int div    & $            $ & 19.97 &    \nparse & 878.23 &    \nparse & 1.93 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-hard-both-t.c.log 
\texttt{hard2     } & int div    & $p           $ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-hard2-both-t.c.log 
\texttt{knuth     } & product    & $            $ & 0.00 &    \nparse & 0.00 &    \nparse & 1.87 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-knuth-both-t.c.log 
\texttt{knuth-nosqrt} &            & $            $ & 7.68 &    \nparse & 893.13 &    \nparse & 133.73 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-knuth-nosqrt-both-t.c.log 
\texttt{lcm1      } & divisor    & $            $ & 0.00 &    \nparse & 8.67 &    \nparse & 10.67 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-lcm1-both-t.c.log 
\texttt{lcm2      } & divisor    & $y           $ & 0.10 &     \rTRUE & 6.71 &    \nparse & 8.78 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-lcm2-both-t.c.log 
\texttt{mannadiv  } &            & $y3          $ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-mannadiv-both-t.c.log 
\texttt{prod4br   } & gcd, lcm   & $b, a        $ & 0.00 &     \rTRUE & 0.00 &    \nparse & \rTO \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-prod4br-both-t.c.log 
\texttt{prodbin   } & gcd, lcm   & $            $ & 0.00 &    \nparse & 0.00 &    \nparse & 2.39 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-prodbin-both-t.c.log 
\texttt{ps2       } & pow sum    & $k + -c      $ & 4.68 &     \rTRUE & 4.98 &     \rTRUE & 11.67 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-ps2-both-t.c.log 
\texttt{ps3       } & pow sum    & $k + -c      $ & 4.32 &     \rTRUE & 8.79 &     \rTRUE & -1.00 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-ps3-both-t.c.log 
\texttt{ps4       } & pow sum    & $k + -c      $ & 4.78 &     \rTRUE & 9.63 &     \rTRUE & -1.00 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-ps4-both-t.c.log 
\texttt{ps5       } & pow sum    & $k + -c      $ & 4.92 &     \rTRUE & 7.36 &     \rTRUE & 14.22 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-ps5-both-t.c.log 
\texttt{ps6       } & pow sum    & $k + -c      $ & 4.77 &     \rTRUE & 28.79 &     \rTRUE & 35.61 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-ps6-both-t.c.log 
\texttt{sqrt1     } & square root & $-c, k + -c  $ & 6.99 &     \rTRUE & 173.88 &     \rTRUE & 183.22 \\ % /svcomp-nla-digbench/out-0WTouHF/dynamo-sqrt1-both-t.c.log 

==> nlaintegrated.tex <==
\texttt{bresenham1} & NT    & NT  & $And(0 == (2\cdot Y\cdot x + -X + 2\cdot Y + -v)\%2,$ & 15.4      \\ 
\texttt{cohencu1  } & NT    & NT  & $(ZConj({-6 <= 6\cdot n + -z}), [          $ & 10.1      \\ 
\texttt{cohencu2  } & NT    & \rUNK & $                                          $ & 24.8      \\ 
\texttt{cohencu3  } & NT    & \rUNK & $                                          $ & 35.9      \\ 
\texttt{cohencu4  } & NT    & \rUNK & $                                          $ & 39.0      \\ 
\texttt{cohencu5  } & NT    & NT  & $(ZConj({-12 == z^{2}  + -12\cdot y + -6\cdot z}), [$ & 10.6      \\ 
\texttt{dijkstra1 } & NT    & \rUNK & $n + -qh, -h, q                            $ & 59.4      \\ 
\texttt{dijkstra2 } & NT    & \rUNK & $n + -qh, r, q                             $ & 353.1     \\ 
\texttt{dijkstra3 } & NT    & \rUNK & $n + -qh, -h, q                            $ & 400.0     \\ 
\texttt{dijkstra4 } & NT    & \rUNK & $n + -qh, q                                $ & 400.0     \\ 
\texttt{dijkstra5 } & NT    & \rUNK & $n + -q-h, h, q                            $ & 400.0     \\ 
\texttt{dijkstra6 } & NT    & \rUNK & $n + -qh, -h, q                            $ & 400.0     \\ 
\texttt{divbin1   } & NT    & \rUNK & $                                          $ & 400.0     \\ 
\texttt{egcd      } & NT    & NT  & $(ZConj({0 == q\cdot x + s\cdot y + -b}), [$ & 85.6      \\ 
\texttt{egcd2     } & NT    & NT  & $(ZConj({0 == p\cdot x + r\cdot y + -a}), [$ & 86.1      \\ 
\texttt{egcd3     } & NT    & NT  & $(ZConj({0 == q\cdot x + s\cdot y + -b}), [$ & 139.2     \\ 
\texttt{fermat1   } & NT    & \rUNK & $k, c, -c, -c + k, -u + -kA + -c, A + -u + c, 2\cdot A + -c, k$ & 400.0     \\ 
\texttt{fermat2   } & NT    & NT  & $(ZConj({0 == u^{2}  + -v^{2}  + -4\cdot A + -4\cdot r + -2\cdot u + 2\cdot v}), [$ & 138.3     \\ 
\texttt{fermat3   } & NT    & NT  & $(ZConj({0 <= u^{2}  + v^{2}  + -4\cdot A + -c + k + -4\cdot r + 2\cdot u + -2\cdot v}), [$ & 400.0     \\ 
\texttt{freire1   } & NT    & \rUNK & $                                          $ & 400.0     \\ 
\texttt{geo1      } & NT    & NT  & $(ZConj({-1 == x\cdot z + -x + -y}), [     $ & 48.5      \\ 
\texttt{geo2      } & NT    & NT  & $(ZConj({-1 == x\cdot z + -y\cdot z + -x}), [$ & 48.6      \\ 
\texttt{geo3      } & NT    & NT  & $(ZConj({0 == a\cdot y\cdot z + -x\cdot z + -a + x}), [$ & 53.2      \\ 
\texttt{hard      } & NT    & NT  & $(ZConj({0 == B\cdot p + -d}), [           $ & 49.2      \\ 
\texttt{hard2     } & NT    & NT  & $(ZConj({0 == B\cdot p + -d}), [           $ & 48.9      \\ 
\texttt{knuth     } & NT    & \rUNK & $                                          $ & 10.6      \\ 
\texttt{knuth-nosqrt} & NT    & NT  & $(ZConj({0 == a\cdot k + -a\cdot t + -d\cdot k + d\cdot t}), [$ & 75.9      \\ 
\texttt{lcm1      } & NT    & NT  & $(ZConj({0 == a\cdot b + -u\cdot x + -v\cdot y}), [$ & 82.9      \\ 
\texttt{lcm2      } & NT    & NT  & $(ZConj({And(0 == a\cdot b + -((u\cdot x + v\cdot y)/2), 0 == (u\cdot x + v\cdot y)\%2)}), [$ & 86.4      \\ 
\texttt{mannadiv  } & NT    & \rUNK & $                                          $ & 197.2     \\ 
\texttt{prod4br   } & NT    & \rUNK & $                                          $ & 198.4     \\ 
\texttt{prodbin   } & NT    & \rUNK & $                                          $ & 337.0     \\ 
\texttt{ps2       } & NT    & NT  & $(ZConj({0 == y^{2}  + -2\cdot x + y}), [  $ & 50.3      \\ 
\texttt{ps3       } & NT    & \rUNK & $                                          $ & 400.0     \\ 
\texttt{ps4       } & NT    & NT  & $(ZConj({0 == y^{4}  + y^{2} \cdot (1 + 2\cdot y) + -4\cdot x}), [$ & 51.4      \\ 
\texttt{ps5       } & NT    & \rUNK & $                                          $ & 61.1      \\ 
\texttt{ps6       } & NT    & \rUNK & $                                          $ & 61.7      \\ 
\texttt{sqrt1     } & NT    & NT  & $(ZConj({-1 == t^{2}  + -4\cdot s + 2\cdot t}), [$ & 51.1      \\ 
\texttt{sqrt2     } & NT    & \rUNK & $-j                                        $ & 400.0     \\ 
\hline
\texttt{cohencu3  } & T     & \rUNK & $-x, k + -z, -y + z, k + -x                $ & 400.0     \\ 
\texttt{cohencu4  } & T     & \rUNK & $                                          $ & 71.1      \\ 
\texttt{cohencu5  } & T     & T   & $-c + k                                    $ & 162.0     \\ 
\texttt{cohencu6  } & T     & \rUNK & $a + -z, a + -n                            $ & 400.0     \\ 
\texttt{cohencu7  } & T     & \rUNK & $a + -n                                    $ & 400.0     \\ 
\texttt{dijkstra1 } & T     & T   & $n + -q                                    $ & 14.2      \\ 
\texttt{dijkstra2 } & T     & \rUNK & $n + -q-c, h, q, -c + k                    $ & 400.0     \\ 
\texttt{dijkstra3 } & T     & \rUNK & $n + -q-c + k                              $ & 400.0     \\ 
\texttt{dijkstra4 } & T     & \rUNK & $n + -q-c + k, h                           $ & 400.0     \\ 
\texttt{dijkstra5 } & T     & \rUNK & $n + -q-c, r, -c + k                       $ & 400.0     \\ 
\texttt{dijkstra6 } & T     & \rUNK & $n + -q-c + k                              $ & 400.0     \\ 
\texttt{divbin1   } & T     & \rUNK & $                                          $ & 2.7       \\ 
\texttt{egcd      } & T     & \rUNK & $a, b                                      $ & 400.0     \\ 
\texttt{egcd2     } & T     & \rUNK & $                                          $ & 2.4       \\ 
\texttt{egcd3     } & T     & \rUNK & $v, c + -v, -v, c + -2\cdot v, c + v, d, -c + 2\cdot v, -c + -v, -d$ & 400.0     \\ 
\texttt{fermat1   } & T     & \rUNK & $-c + k                                    $ & 400.0     \\ 
\texttt{freire1   } & T     & \rUNK & $                                          $ & 400.0     \\ 
\texttt{geo1      } & T     & \rUNK & $y, -c + -x, k + -c                        $ & 400.0     \\ 
\texttt{geo2      } & T     & \rUNK & $k + -c                                    $ & 400.0     \\ 
\texttt{geo3      } & T     & \rUNK & $-y, y, -x, x, -c + -x, k + -c             $ & 400.0     \\ 
\texttt{hard      } & T     & \rUNK & $                                          $ & 3.6       \\ 
\texttt{hard2     } & T     & \rUNK & $                                          $ & 400.0     \\ 
\texttt{knuth     } & T     & \rUNK & $                                          $ & 3.7       \\ 
\texttt{knuth-nosqrt} & T     & \rUNK & $                                          $ & 400.0     \\ 
\texttt{lcm1      } & T     & \rUNK & $                                          $ & 400.0     \\ 
\texttt{lcm2      } & T     & \rUNK & $x, y                                      $ & 400.0     \\ 
\texttt{mannadiv  } & T     & \rUNK & $y3                                        $ & 400.0     \\ 
\texttt{prod4br   } & T     & \rUNK & $q, -q, b, a                               $ & 400.0     \\ 
\texttt{prodbin   } & T     & \rUNK & $                                          $ & 1.9       \\ 
\texttt{ps2       } & T     & T   & $k + -c                                    $ & 22.3      \\ 
\texttt{ps3       } & T     & T   & $k + -c                                    $ & 14.2      \\ 
\texttt{ps4       } & T     & T   & $-c, c + -x, k + -c                        $ & 29.5      \\ 
\texttt{ps5       } & T     & T   & $k + -c                                    $ & 16.8      \\ 
\texttt{ps6       } & T     & T   & $k + -c                                    $ & 68.8      \\ 
\texttt{sqrt1     } & T     & T   & $-c, k + -c                                $ & 194.9     \\ 

==> nlaintegrated2.tex <==
\texttt{cohencu3  } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{cohencu4  } & T  &        & 7.7 & \rUNK    &   71.1 \\ 
\texttt{cohencu5  } & T  & \gRF   & 7.1 & T        &  162.0 \\ 
\texttt{cohencu6  } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{cohencu7  } & T  & \gRF   & 0.0 & \rUNK    &  400.0 \\ 
\texttt{dijkstra1 } & T  & \gRF   & 0.0 & T        &   14.2 \\ 
\texttt{dijkstra2 } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra3 } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra4 } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra5 } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra6 } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{divbin1   } & T  &        & \rUNK & \rUNK    &    2.7 \\ 
\texttt{egcd      } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{egcd2     } & T  &        & \rUNK & \rUNK    &    2.4 \\ 
\texttt{egcd3     } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{fermat1   } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{freire1   } & T  &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{geo1      } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{geo2      } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{geo3      } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{hard      } & T  &        & \rUNK & \rUNK    &    3.6 \\ 
\texttt{hard2     } & T  &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{knuth     } & T  &        & \rUNK & \rUNK    &    3.7 \\ 
\texttt{knuth-nosqrt} & T  &        & 0.1 & \rUNK    &  400.0 \\ 
\texttt{lcm1      } & T  &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{lcm2      } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{mannadiv  } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{prod4br   } & T  & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{prodbin   } & T  &        & \rUNK & \rUNK    &    1.9 \\ 
\texttt{ps2       } & T  & \gRF   & 8.5 & T        &   22.3 \\ 
\texttt{ps3       } & T  & \gRF   & 4.8 & T        &   14.2 \\ 
\texttt{ps4       } & T  & \gRF   & 9.9 & T        &   29.5 \\ 
\texttt{ps5       } & T  & \gRF   & 4.8 & T        &   16.8 \\ 
\texttt{ps6       } & T  & \gRF   & 4.6 & T        &   68.8 \\ 
\texttt{sqrt1     } & T  & \gRF   & 10.1 & T        &  194.9 \\ 
\texttt{bresenham1} & NT &  \gRS  & \rUNK & NT       &   15.4 \\ 
\texttt{cohencu1  } & NT &  \gRS  & \rUNK & NT       &   10.1 \\ 
\texttt{cohencu2  } & NT &        & \rUNK & \rUNK    &   24.8 \\ 
\texttt{cohencu3  } & NT &        & 0.0 & \rUNK    &   35.9 \\ 
\texttt{cohencu4  } & NT &        & 0.0 & \rUNK    &   39.0 \\ 
\texttt{cohencu5  } & NT &  \gRS  & \rUNK & NT       &   10.6 \\ 
\texttt{dijkstra1 } & NT & \gRF   & 0.0 & \rUNK    &   59.4 \\ 
\texttt{dijkstra2 } & NT & \gRF   & \rUNK & \rUNK    &  353.1 \\ 
\texttt{dijkstra3 } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra4 } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra5 } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{dijkstra6 } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{divbin1   } & NT &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{egcd      } & NT &  \gRS  & \rUNK & NT       &   85.6 \\ 
\texttt{egcd2     } & NT &  \gRS  & \rUNK & NT       &   86.1 \\ 
\texttt{egcd3     } & NT &  \gRS  & \rUNK & NT       &  139.2 \\ 
\texttt{fermat1   } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 
\texttt{fermat2   } & NT &  \gRS  & \rUNK & NT       &  138.3 \\ 
\texttt{fermat3   } & NT & \gRF \gRS & 26.8 & NT       &  400.0 \\ 
\texttt{freire1   } & NT &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{geo1      } & NT &  \gRS  & \rUNK & NT       &   48.5 \\ 
\texttt{geo2      } & NT &  \gRS  & \rUNK & NT       &   48.6 \\ 
\texttt{geo3      } & NT &  \gRS  & \rUNK & NT       &   53.2 \\ 
\texttt{hard      } & NT &  \gRS  & \rUNK & NT       &   49.2 \\ 
\texttt{hard2     } & NT &  \gRS  & \rUNK & NT       &   48.9 \\ 
\texttt{knuth     } & NT &        & \rUNK & \rUNK    &   10.6 \\ 
\texttt{knuth-nosqrt} & NT &  \gRS  & \rUNK & NT       &   75.9 \\ 
\texttt{lcm1      } & NT &  \gRS  & \rUNK & NT       &   82.9 \\ 
\texttt{lcm2      } & NT &  \gRS  & \rUNK & NT       &   86.4 \\ 
\texttt{mannadiv  } & NT &        & 0.0 & \rUNK    &  197.2 \\ 
\texttt{prod4br   } & NT &        & 0.0 & \rUNK    &  198.4 \\ 
\texttt{prodbin   } & NT &        & 0.0 & \rUNK    &  337.0 \\ 
\texttt{ps2       } & NT &  \gRS  & \rUNK & NT       &   50.3 \\ 
\texttt{ps3       } & NT &        & \rUNK & \rUNK    &  400.0 \\ 
\texttt{ps4       } & NT &  \gRS  & \rUNK & NT       &   51.4 \\ 
\texttt{ps5       } & NT &        & \rUNK & \rUNK    &   61.1 \\ 
\texttt{ps6       } & NT &        & \rUNK & \rUNK    &   61.7 \\ 
\texttt{sqrt1     } & NT &  \gRS  & \rUNK & NT       &   51.1 \\ 
\texttt{sqrt2     } & NT & \gRF   & \rUNK & \rUNK    &  400.0 \\ 

==> termcraftlitnt.tex <==
BrMaSi-CAV2005-Fig1-mod.c           & $ y1, y2          $ & 7.5  & \rTRUE & 4.8  & \rUNK  &  15.8 &   1.7 &   \ULTIMATE{  0.1   & \rFALSE } \\

ChCoFuNiHe-TACAS2014-Intro.c        & $ i, 3 + -i, 4 + -i  $ & 0.7  & \rTRUE & 3.9  & \rUNK  &  9.42 &   1.1 &   \ULTIMATE{  0.2   & \rFALSE } \\
Velroyen.c                          & $ x, -x           $ & 0.9  & \rTRUE & 8.6  & \rUNK  &  12.1 &   0.7 &   \ULTIMATE{  2.2   & \rFALSE } \\

